Gromov-Wasserstein Autoencoders

Variational Autoencoder (VAE)-based generative models offer flexible representation learning by incorporating meta-priors, general premises considered beneficial for downstream tasks. However, the incorporated meta-priors often involve ad-hoc model deviations from the original likelihood architecture, causing undesirable changes in their training. In this paper, we propose a novel representation learning method, Gromov-Wasserstein Autoencoders (GWAE), which directly matches the latent and data distributions using the variational autoencoding scheme. Instead of likelihood-based objectives, GWAE models minimize the Gromov-Wasserstein (GW) metric between the trainable prior and given data distributions. The GW metric measures the distance structure-oriented discrepancy between distributions even with different dimensionalities, which provides a direct measure between the latent and data spaces. By restricting the prior family, we can introduce meta-priors into the latent space without changing their objective. The empirical comparisons with VAE-based models show that GWAE models work in two prominent meta-priors, disentanglement and clustering, with their GW objective unchanged.

==> s45_discussions.tex <==
\textbf{Broader Impacts.}
Representation learning on real-world data alleviates the burden of labor-intensive annotation and expands the application of machine learning to real-world data.
Representations obtained without supervisory signals can reveal the structure and origins of data, facilitating big data analysis and knowledge discovery.
However, as with other unsupervised algorithms, an application to real-world decision-making processes must be carefully conducted, since data biases may affect the results.
Representation learning without prior information may directly reflect biases and prejudices and may lead to privacy violations.
Future work will consider the calls for these problems, such as debiasing, anonymization, and explainable inference.

\textbf{Limitations.}
One major limitation inherited from existing representation learning methods is the performance dependence on the choice of the hyperparameters consisting of the value of the Lagrange multipliers and the prior class~(meta-prior).
Therefore, model performance verification relies on computationally expensive hyperparameter optimization using empirical evaluations.
This issue is attributed to applying SGD to multi-objective optimization in large-scale data.
Hence, converting conditions into a model structure may alleviate potential trade-offs between objectives.
For example, modifying the autoencoding scheme~(\eg, using graph convolutional networks) in addition to the prior, can be a good remedy.
Inductive biases, such as weak supervision and domain knowledge, are also solutions for real applications with specific domains~\cite{Locatello2019}.
